How to Work with Honest but Curious Judges? (Preliminary Report)

The three-judges protocol, recently advocated by Mclver and Morgan as an example of stepwise refinement of security protocols, studies how to securely compute the majority function to reach a final verdict without revealing each individual judge's decision. We extend their protocol in two different ways for an arbitrary number of 2n+1 judges. The first generalisation is inherently centralised, in the sense that it requires a judge as a leader who collects information from others, computes the majority function, and announces the final result. A different approach can be obtained by slightly modifying the well-known dining cryptographers protocol, however it reveals the number of votes rather than the final verdict. We define a notion of conditional anonymity in order to analyse these two solutions. Both of them have been checked in the model checker MCMAS.

==> eptcsdata.tex <==
\providecommand{\event}{M. Boreale, S. Kremer (Eds.):\\
 Security Issues in Concurrency (SecCo'09)}
\providecommand{\volume}{7}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{31}
\providecommand{\eid}{3}

